BayesCPF: Enabling Collective Perception in Robot Swarms with Degrading Sensors

The collective perception problem -- where a group of robots perceives its surroundings and comes to a consensus on an environmental state -- is a fundamental problem in swarm robotics. Past works studying collective perception use either an entire robot swarm with perfect sensing or a swarm with only a handful of malfunctioning members. A related study proposed an algorithm that does account for an entire swarm of unreliable robots but assumes that the sensor faults are known and remain constant over time. To that end, we build on that study by proposing the Bayes Collective Perception Filter (BayesCPF) that enables robots with continuously degrading sensors to accurately estimate the fill ratio -- the rate at which an environmental feature occurs. Our main contribution is the Extended Kalman Filter within the BayesCPF, which helps swarm robots calibrate for their time-varying sensor degradation. We validate our method across different degradation models, initial conditions, and environments in simulated and physical experiments. Our findings show that, regardless of degradation model assumptions, fill ratio estimation using the BayesCPF is competitive to the case if the true sensor accuracy is known, especially when assumptions regarding the model and initial sensor accuracy levels are preserved.

==> acknowledgments.tex <==
\section{Acknowledgment}
This research was performed using computational resources supported by the Academic \& Research Computing group at Worcester Polytechnic Institute. This work was partially supported by the DEVCOM Analysis Center and was accomplished under Cooperative Agreement Number W911NF-22-2-0001. The views and conclusions contained in this document are those of the authors and should not be interpreted as representing the official policies, either expressed or implied, of the Army Research Office or the U.S. Government. The U.S. Government is authorized to reproduce and distribute reprints for Government purposes notwithstanding any copyright notation herein.

==> figures/bayes_cpf_variables.tex <==
\newcommand{\robotimodulefontsize}{10pt}
\newcommand{\robotjmodulefontsize}{7pt}
\newcommand{\insetrobotlabelfontsize}{8pt}
\newcommand{\variablesfontsize}{9pt}
\newcommand{\robotititlefontsize}{13pt}
\newcommand{\robotjtitlefontsize}{10pt}

==> figures/heatmap_variables.tex <==
\newcommand{\xlabelfontsize}{6pt}
\newcommand{\ylabelfontsize}{\xlabelfontsize}
\newcommand{\xlabeltitlefontsize}{8pt}
\newcommand{\ylabeltitlefontsize}{\xlabeltitlefontsize}
\newcommand{\zlabelfontsize}{6pt}
\newcommand{\zlabeltitlefontsize}{6pt}

==> figures/multix_boxplot_variables.tex <==
\newcommand{\xmajorlabelfontsize}{7pt}
\newcommand{\xminorlabelfontsize}{6pt} % x2 label
\newcommand{\rowlabelfontsize}{10pt} % eta labels
\newcommand{\columnlabelfontsize}{10pt} % Transient vs Equilibrium labels
\newcommand{\ylabelfontsize}{6pt} % y label
\newcommand{\ylabeltitlefontsize}{\xmajorlabelfontsize} % y label title
\newcommand{\xminorlabelvspace}{-8pt} % spacing for the x minor label
\newcommand{\legendtitlefontsize}{8pt} % legend title font size
\newcommand{\legendlabelfontsize}{7pt} % legend label font size
\newcommand{\legendtitlehspace}{0pt} % horizontal spacing for legend title
\newcommand{\legendlabelhspace}{-1pt} % horizontal spacing for legend labels
\newcommand{\squarexmajorlabelfontsize}{7pt}
\newcommand{\squarexminorlabelfontsize}{6pt} % x2 label
\newcommand{\squarerowlabelfontsize}{10pt} % left-side labels
\newcommand{\squarecolumnlabelfontsize}{10pt} % Transient vs Equilibrium labels
\newcommand{\squareylabelfontsize}{6pt} % y label
\newcommand{\squareylabeltitlefontsize}{\xmajorlabelfontsize} % y label title
\newcommand{\squarexminorlabelvspace}{-10pt} % spacing for the x minor label
% 1.79857e-3 is the raised distance for the secondary x-axis labels

==> figures/time_series_variables.tex <==
\newcommand{\xlabelfontsize}{8pt}
\newcommand{\ylabelfontsize}{\xlabelfontsize}
\newcommand{\xlabeltitlefontsize}{9pt}
\newcommand{\ylabeltitlefontsize}{\xlabeltitlefontsize}
\newcommand{\internaltextfontsize}{8pt}
\newcommand{\dualcolxlabelfontsize}{6pt}
\newcommand{\dualcolylabelfontsize}{\dualcolxlabelfontsize}
\newcommand{\dualcolxlabeltitlefontsize}{6.5pt}
\newcommand{\dualcolylabeltitlefontsize}{\dualcolxlabeltitlefontsize}
